Do Chess Explanations Reflect Model Decisions? Behavioral and Token-Level Tests of LLM Reasoning Faithfulness

Large language models can produce fluent explanations for chess moves, but plausible language does not necessarily reflect the reasoning behind a decision. We study this question in chess, where the board state is fully observable, legal actions can be enumerated, and move quality can be evaluated independently. Across 200 Lichess endgame puzzles, we test explanations using move recoverability, decoder-side controls, and token-level scoring of legal candidate moves. Unmasked explanations make generated moves easy to recover, but this advantage drops sharply after explicit move hints are removed. Under strict masking, explanations provide only small and decoder-dependent gains over the board state alone. Token-level scoring shows that explanations can nevertheless alter move preferences: random but plausible explanations from other puzzles reduce the probability of the correct move, indicating that irrelevant reasoning text is not simply ignored. We also find that recognizable endgame motifs can make generated moves easier to recover without reliably improving move correctness. Together, these results show that linguistic plausibility, consistency with a generated action, and solution correctness are distinct properties. Fluent chess explanations can influence action preferences and support a coherent move narrative while providing only limited evidence of faithful reasoning.

==> tables/counterfactual_sensitivity.tex <==
\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lc}
\toprule
Metric & Value \\
\midrule
Mean explanation similarity & 0.203 \\
Generated move changed & 0.959 \\
Top-prob move changed & 1.000 \\
Recoverability predicted move changed & 0.816 \\
Recoverability match changed & 0.000 \\
\bottomrule
\end{tabular}
\caption{Counterfactual sensitivity summary on 25 puzzles (Mistral-7B). Values are fraction of variants where a change occurred, except explanation similarity (SequenceMatcher ratio).}
\label{tab:counterfactual_sensitivity}
\end{table}


==> tables/decoder_controls_groq.tex <==
\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{llccccc}
\toprule
Decoder & Condition & Parsed & Generated@1 & Generated@3 & Reference@1 & Reference@3 \\
\midrule
Llama-3.3-70B & FEN only & 0.510 & 0.047 & 0.060 & 0.000 & 0.000 \\
 & Explanation only & 0.201 & 0.000 & 0.020 & 0.000 & 0.007 \\
 & Strict mask & 0.436 & 0.073 & 0.100 & 0.053 & 0.053 \\
 & Maximal mask & 0.423 & 0.073 & 0.073 & 0.060 & 0.060 \\
 & Random expl. & 0.376 & 0.007 & 0.013 & 0.000 & 0.007 \\
 & Unmasked & 0.879 & 0.680 & 0.740 & 0.113 & 0.147 \\
\midrule
Qwen3-32B & FEN only & 0.376 & 0.007 & 0.007 & 0.007 & 0.020 \\
 & Explanation only & 0.121 & 0.000 & 0.007 & 0.007 & 0.007 \\
 & Strict mask & 0.369 & 0.020 & 0.033 & 0.020 & 0.027 \\
 & Maximal mask & 0.450 & 0.027 & 0.027 & 0.027 & 0.027 \\
 & Random expl. & 0.389 & 0.013 & 0.020 & 0.013 & 0.013 \\
 & Unmasked & 0.826 & 0.737 & 0.743 & 0.113 & 0.113 \\
\bottomrule
\end{tabular}
\caption{Decoder-side controls on the same 50-puzzle subset, pooled across prompt styles. Parsed is the rate at which the decoder returned at least one extractable move. Qwen3 uses hidden/no-reasoning mode.}
\label{tab:decoder_controls_groq}
\end{table*}


==> tables/decoder_controls_groq_parsed_only.tex <==
\begin{table*}[t]
\centering
\scriptsize
\begin{tabular}{llccccc}
\toprule
Decoder & Condition & Parsed $n$ & Generated@1 & Generated@3 & Reference@1 & Reference@3 \\
\midrule
Llama-3.3-70B & FEN only & 76 & 0.092 & 0.118 & 0.000 & 0.000 \\
 & Explanation only & 30 & 0.000 & 0.100 & 0.000 & 0.033 \\
 & Strict mask & 65 & 0.169 & 0.231 & 0.123 & 0.123 \\
 & Maximal mask & 63 & 0.175 & 0.175 & 0.143 & 0.143 \\
 & Random expl. & 56 & 0.018 & 0.036 & 0.000 & 0.018 \\
 & Unmasked & 131 & 0.779 & 0.847 & 0.130 & 0.168 \\
\midrule
Qwen3-32B & FEN only & 56 & 0.018 & 0.018 & 0.018 & 0.054 \\
 & Explanation only & 18 & 0.000 & 0.056 & 0.056 & 0.056 \\
 & Strict mask & 55 & 0.055 & 0.091 & 0.055 & 0.073 \\
 & Maximal mask & 67 & 0.060 & 0.060 & 0.060 & 0.060 \\
 & Random expl. & 58 & 0.034 & 0.052 & 0.034 & 0.034 \\
 & Unmasked & 123 & 0.894 & 0.902 & 0.138 & 0.138 \\
\bottomrule
\end{tabular}
\caption{Parsed-only decoder controls on the 50-puzzle subset, pooled across prompt styles. Rates condition on at least one extracted UCI move; end-to-end rates appear in Table~\ref{tab:decoder_controls_groq}.}
\label{tab:decoder_controls_groq_parsed}
\end{table*}


==> tables/decoder_recoverability_200.tex <==
\begin{table*}[t]
\centering
\scriptsize
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccc}
\toprule
Decoder & Prompt & Parsed & Generated@1 & Generated@3 & Reference@1 & Reference@3 \\
\midrule
GPT-4.1-mini & Brief & 0.955 [0.925,0.980] & 0.392 [0.325,0.464] & 0.510 [0.438,0.577] & 0.055 [0.025,0.090] & 0.095 [0.060,0.135] \\
GPT-4.1-mini & Calculation & 0.975 [0.950,0.995] & 0.379 [0.313,0.446] & 0.462 [0.390,0.533] & 0.055 [0.025,0.085] & 0.100 [0.060,0.145] \\
GPT-4.1-mini & Teaching & 0.985 [0.965,1.000] & 0.387 [0.322,0.452] & 0.497 [0.427,0.568] & 0.090 [0.055,0.135] & 0.135 [0.090,0.185] \\
Llama-3.3-70B & Brief & 0.995 [0.985,1.000] & 0.067 [0.036,0.103] & 0.129 [0.088,0.180] & 0.010 [0.000,0.025] & 0.035 [0.010,0.065] \\
Llama-3.3-70B & Calculation & 1.000 [1.000,1.000] & 0.077 [0.041,0.118] & 0.128 [0.082,0.179] & 0.005 [0.000,0.015] & 0.030 [0.010,0.055] \\
Llama-3.3-70B & Teaching & 1.000 [1.000,1.000] & 0.075 [0.040,0.116] & 0.126 [0.080,0.176] & 0.025 [0.005,0.050] & 0.045 [0.020,0.075] \\
Qwen3-32B & Brief & 0.940 [0.905,0.970] & 0.057 [0.026,0.093] & 0.077 [0.041,0.119] & 0.010 [0.000,0.025] & 0.020 [0.005,0.040] \\
Qwen3-32B & Calculation & 0.950 [0.920,0.980] & 0.097 [0.056,0.138] & 0.159 [0.108,0.210] & 0.015 [0.000,0.035] & 0.040 [0.015,0.070] \\
Qwen3-32B & Teaching & 0.960 [0.930,0.985] & 0.060 [0.030,0.095] & 0.106 [0.060,0.146] & 0.020 [0.005,0.040] & 0.035 [0.010,0.065] \\
\bottomrule
\end{tabular}
}
\caption{Strict-mask move recoverability on 200 puzzles. Unparsed decoder outputs count as failures; brackets show puzzle-bootstrap 95\% confidence intervals.}
\label{tab:decoder_recoverability_200}
\end{table*}


==> tables/decoder_recoverability_200_parsed.tex <==
\begin{table*}[t]
\centering
\scriptsize
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccc}
\toprule
Decoder & Prompt & Parsed & Generated@1 & Generated@3 & Reference@1 & Reference@3 \\
\midrule
GPT-4.1-mini & Brief & 1.000 [1.000,1.000] & 0.398 [0.330,0.466] & 0.518 [0.450,0.592] & 0.058 [0.026,0.089] & 0.099 [0.058,0.147] \\
GPT-4.1-mini & Calculation & 1.000 [1.000,1.000] & 0.379 [0.313,0.446] & 0.462 [0.390,0.533] & 0.056 [0.026,0.087] & 0.103 [0.062,0.149] \\
GPT-4.1-mini & Teaching & 1.000 [1.000,1.000] & 0.391 [0.325,0.462] & 0.503 [0.431,0.574] & 0.091 [0.056,0.137] & 0.137 [0.091,0.188] \\
Llama-3.3-70B & Brief & 1.000 [1.000,1.000] & 0.067 [0.031,0.104] & 0.130 [0.083,0.181] & 0.010 [0.000,0.025] & 0.035 [0.015,0.065] \\
Llama-3.3-70B & Calculation & 1.000 [1.000,1.000] & 0.077 [0.041,0.118] & 0.128 [0.082,0.179] & 0.005 [0.000,0.015] & 0.030 [0.010,0.055] \\
Llama-3.3-70B & Teaching & 1.000 [1.000,1.000] & 0.075 [0.040,0.116] & 0.126 [0.080,0.176] & 0.025 [0.005,0.050] & 0.045 [0.020,0.075] \\
Qwen3-32B & Brief & 1.000 [1.000,1.000] & 0.060 [0.027,0.098] & 0.082 [0.044,0.126] & 0.011 [0.000,0.027] & 0.021 [0.005,0.043] \\
Qwen3-32B & Calculation & 1.000 [1.000,1.000] & 0.103 [0.065,0.146] & 0.168 [0.119,0.222] & 0.016 [0.000,0.037] & 0.042 [0.016,0.074] \\
Qwen3-32B & Teaching & 1.000 [1.000,1.000] & 0.063 [0.031,0.099] & 0.110 [0.068,0.157] & 0.021 [0.005,0.042] & 0.036 [0.010,0.068] \\
\bottomrule
\end{tabular}
}
\caption{Parsed-only strict-mask recoverability on 200 puzzles. Rates are conditional on extracting at least one UCI move.}
\label{tab:decoder_recoverability_200_parsed}
\end{table*}


==> tables/elfen_human_llm_features.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lrrrr}
\toprule
Feature & LLM & Human & $\Delta$ & $q$ \\
\midrule
Adverbs & 1.61 & 7.29 & -0.92 & $<.001$ \\
Pronouns & 3.19 & 7.22 & -0.79 & $<.001$ \\
Hedges & 1.54 & 4.30 & -0.67 & $<.001$ \\
Tokens/sentence & 36.04 & 16.43 & 0.77 & $<.001$ \\
tree depth & 6.80 & 3.58 & 0.78 & $<.001$ \\
Determiners & 6.67 & 3.66 & 0.74 & $<.001$ \\
Nouns & 9.98 & 6.07 & 0.74 & $<.001$ \\
Gunning fog & 17.35 & 7.81 & 0.83 & $<.001$ \\
\bottomrule
\end{tabular}
\caption{Exploratory ELFEN comparison of 50-word LLM explanation chunks and five human chess-reasoning transcript sources. $\Delta$ is Cliff's delta, positive when the feature is larger in LLM text. $q$ is Benjamini--Hochberg corrected.}
\label{tab:elfen_human_llm}
\end{table}


==> tables/endgame_summary.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{lrrrrrr}
\toprule
Endgame type & Puzzles & Legal & Exact & Gen.\ rec. & Ref.\ rec. & Motif mention \\
\midrule
Pawn & 40 & .558 & .133 & .483 & .125 & .775 \\
Rook & 56 & .467 & .103 & .494 & .062 & .788 \\
Knight & 10 & .700 & .067 & .233 & .033 & .867 \\
Bishop & 14 & .300 & .025 & .256 & .026 & .600 \\
Queen$^\dagger$ & 7 & .810 & .190 & .238 & .143 & 1.000 \\
Queen--rook & 65 & .558 & .037 & .323 & .053 & .979 \\
Bishop--knight$^\dagger$ & 7 & .211 & .000 & .263 & .000 & .579 \\
Bishop vs.\ pawns$^\dagger$ & 1 & 1.000 & .667 & .333 & .000 & 1.000 \\
\bottomrule
\end{tabular}
\caption{Endgame-type analysis over the three GPT-4.1-mini prompt conditions. Recoverability is top-1. $^\dagger$Fewer than ten puzzles; descriptive only.}
\label{tab:endgame_summary}
\end{table*}


==> tables/engine_clean_summary.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{lcccc}
\toprule
Prompt & Legal (95\% CI) & Exact (95\% CI) & Median loss, legal & Mean loss, all \\
\midrule
Brief & .535 [.470,.605] & .080 [.045,.120] & 471 & 1244.8 \\
Calculation & .415 [.350,.480] & .070 [.035,.110] & 459 & 1397.8 \\
Teaching & .585 [.515,.655] & .095 [.055,.140] & 463 & 1157.7 \\
\bottomrule
\end{tabular}
\caption{GPT-4.1-mini move quality on 200 puzzles. Engine loss is clipped at 2000 centipawns. ``Legal'' loss excludes illegal and unparsed outputs; ``all'' assigns them the 2000-centipawn cap. Exact match is measured over all outputs.}
\label{tab:engine_clean}
\end{table*}


==> tables/groq_200_prompt_summary.tex <==
\begin{table*}[t]
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{l l c c c c c c c}
\toprule
Model & Prompt & $n$ & Parsed & Legal & Exact & Avg $\Delta$ (cp) & Avg words & Avg spec. \\
\midrule
gpt-4.1-mini & brief & 200 & 0.970 & 0.535 & 0.080 & 11559.5 & 44.4 & 0.201 \\
gpt-4.1-mini & calc & 200 & 0.975 & 0.415 & 0.070 & 12364.2 & 146.1 & 0.321 \\
gpt-4.1-mini & teaching & 200 & 0.995 & 0.585 & 0.095 & 12304.3 & 117.4 & 0.205 \\
llama-3.1-8b-instant & brief & 200 & 0.960 & 0.015 & 0.005 & 66600.3 & 47.2 & 0.256 \\
llama-3.1-8b-instant & calc & 200 & 0.270 & 0.070 & 0.010 & 21781.6 & 200.7 & 0.231 \\
llama-3.1-8b-instant & teaching & 200 & 0.990 & 0.030 & 0.005 & 50084.5 & 194.1 & 0.230 \\
llama-3.3-70b-versatile & brief & 200 & 0.250 & 0.045 & 0.000 & 22378.6 & 36.8 & 0.131 \\
llama-3.3-70b-versatile & calc & 200 & 0.630 & 0.100 & 0.010 & 5283.1 & 174.9 & 0.209 \\
llama-3.3-70b-versatile & teaching & 200 & 0.555 & 0.060 & 0.005 & 16795.8 & 162.8 & 0.145 \\
meta-llama/llama-4-scout-17b-16e-instruct & brief & 200 & 0.730 & 0.100 & 0.005 & 20339.7 & 77.4 & 0.210 \\
meta-llama/llama-4-scout-17b-16e-instruct & calc & 200 & 0.500 & 0.035 & 0.000 & 28948.4 & 163.7 & 0.151 \\
meta-llama/llama-4-scout-17b-16e-instruct & teaching & 200 & 0.850 & 0.045 & 0.000 & 11368.6 & 195.7 & 0.201 \\
moonshotai/kimi-k2-instruct-0905 & brief & 200 & 0.860 & 0.505 & 0.080 & 14197.0 & 47.1 & 0.442 \\
moonshotai/kimi-k2-instruct-0905 & calc & 200 & 0.880 & 0.520 & 0.060 & 13774.0 & 125.7 & 0.477 \\
moonshotai/kimi-k2-instruct-0905 & teaching & 200 & 0.850 & 0.435 & 0.075 & 16462.0 & 118.6 & 0.319 \\
qwen/qwen3-32b & brief & 200 & 0.075 & 0.060 & 0.010 & 8571.2 & 144.6 & 0.264 \\
qwen/qwen3-32b & calc & 200 & 0.040 & 0.020 & 0.005 & 25397.5 & 138.4 & 0.214 \\
qwen/qwen3-32b & teaching & 200 & 0.065 & 0.065 & 0.005 & 7983.1 & 152.0 & 0.244 \\
\bottomrule
\end{tabular}
}
\caption{Model comparison on 200 Lichess endgame puzzles. Parsed = fraction of outputs where a move could be extracted.}
\label{tab:groq_prompt_summary}
\end{table*}


==> tables/hosted_model_summary.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{lccccc}
\toprule
Model & Parsed & Legal & Exact & Avg. words & Avg. specificity \\
\midrule
GPT-4.1-mini & 0.980 & 0.512 & 0.082 & 102.6 & 0.242 \\
Llama-3.1-8B-Instant & 0.740 & 0.038 & 0.007 & 147.3 & 0.239 \\
Llama-3.3-70B-Versatile & 0.478 & 0.068 & 0.005 & 124.8 & 0.162 \\
Llama-4-Scout-17B & 0.693 & 0.060 & 0.002 & 145.6 & 0.187 \\
Kimi-K2-Instruct & 0.863 & 0.487 & 0.072 & 97.1 & 0.413 \\
Qwen3-32B & 0.060 & 0.048 & 0.007 & 145.0 & 0.241 \\
\bottomrule
\end{tabular}
\caption{Hosted-model results averaged across brief, calculation, and teaching prompts on 200 puzzles. The full 18-condition table is reported in Appendix~\ref{tab:groq_prompt_summary}.}
\label{tab:hosted_model_summary}
\end{table*}


==> tables/human_book4_reasoning_summary.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{lrrrrrrr}
\toprule
Group & $n$ & Correct & Words & Squares & Cond. & Line depth & Spec. \\
\midrule
Human pre-solution & 3 & 0.50 & 560.0 & 35.0 & 27.3 & 5.3 & 0.299 \\
Human post-solution & 3 & 1.00 & 209.7 & 21.7 & 6.7 & 7.7 & 0.606 \\
LLM brief & 4 & 0.50 & 47.5 & 1.5 & 0.0 & 1.3 & 0.152 \\
LLM calculation & 4 & 0.00 & 128.3 & 7.5 & 1.5 & 3.5 & 0.290 \\
LLM teaching & 4 & 0.00 & 126.0 & 6.8 & 0.8 & 2.3 & 0.226 \\
\bottomrule
\end{tabular}
\caption{Pilot comparison of human think-aloud reasoning and LLM explanations on book pawn endings. Human pre-solution rows are spontaneous solving attempts; post-solution rows are explanations after seeing the book line.}
\label{tab:human_book4_reasoning}
\end{table*}


==> tables/human_commentary_segment_comparison.tex <==
\begin{table*}[h]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{llrrrrrrr}
\toprule
Source & Type & Seg. & Words & Coord. & Move & Spatial & Concept & Spec. \\
\midrule
Book-A & Human ctrl. & 383 & 7.6 & 0.256 & 0.258 & 0.308 & 0.157 & 0.353 \\
Book-B & Human ctrl. & 521 & 7.5 & 0.048 & 0.050 & 0.482 & 0.111 & 0.094 \\
Book-C & Human ctrl. & 253 & 10.2 & 0.079 & 0.079 & 0.530 & 0.154 & 0.232 \\
YouTube-J & Human nat. & 73 & 29.0 & 0.151 & 0.151 & 0.986 & 0.521 & 0.056 \\
YouTube-S & Human nat. & 344 & 15.6 & 0.140 & 0.140 & 0.948 & 0.631 & 0.136 \\
LLM-brief & LLM & 6299 & 12.6 & 0.326 & 0.389 & 0.217 & 0.177 & 0.728 \\
LLM-calc & LLM & 17895 & 10.6 & 0.292 & 0.387 & 0.174 & 0.179 & 0.415 \\
LLM-teach & LLM & 13826 & 13.6 & 0.389 & 0.430 & 0.336 & 0.176 & 0.458 \\
\bottomrule
\end{tabular}
\caption{Segment-level reasoning-style markers for human and LLM chess explanations. Book-A--C are controlled think-aloud transcripts from three participants solving pawn-ending book puzzles; YouTube-J and YouTube-S are public puzzle-solving commentaries; LLM rows pool six model families by prompting style. All rows use the same feature extractor. Human rows use ASR segments and LLM rows use sentence-like units, so the comparison is descriptive rather than a matched human-performance baseline. Coord., Move, Spatial, and Concept report the proportion of units containing explicit coordinates, move notation, deictic or positional board language, or tactical and strategic vocabulary. Spec. is the normalized text-only specificity score.}
\label{tab:human_llm_reasoning_segments}
\end{table*}


==> tables/human_llm_examples.tex <==
\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{@{}p{0.27\columnwidth}p{0.64\columnwidth}@{}}
\toprule
Source and outcome & Selected excerpt \\
\midrule
Puzzle 2, human; incorrect final answer &
``If we were to play king to d6, then we might have h5, c5, h4, c6 \ldots and then both make a queen. This might actually be a draw, so this shouldn't be right. Okay, so we can't run immediately.'' \\
\addlinespace
Puzzle 1/2, Book-B participant; concrete but wrong candidate &
``The first movement is to move the pawn from c3 into c4. \ldots I prefer to keep the king at the corner because I want to bring the white king into also corner.'' \\
\addlinespace
Puzzle 1/2, Book-C participant; schema-level plan &
``The goal of white can really probably win by promotion \ldots black wants to do is kind of just be in front of this pawn.'' \\
\addlinespace
Puzzle 2, model; \texttt{Kc7}, incorrect &
``White plays c7, pushing the pawn closer to promotion. \ldots White's king on c6 supports the pawn on c7, which is one step away from queening. \ldots Therefore, c6c7 is the winning move.'' \\
\midrule
Puzzle 4, human; unresolved &
``We can't stop this pawn from queening, I don't think so. And if a queen lands here then that also attacks our promotion square. So we might need to set it up so that our king protects that.'' \\
\addlinespace
Puzzle 4, model; \texttt{h4}, reference move &
``White should push the pawn to h4 to start advancing it towards promotion. Black's king is too far to stop the pawn \ldots This move initiates a winning plan for White.'' \\
\bottomrule
\end{tabular}
\caption{Qualitative examples from the controlled pawn-ending pilot. Human rows are think-aloud excerpts from the participants; model rows are generated explanations. Puzzle~4 is a drawing study: the model selects the reference move but incorrectly describes it as winning. Excerpts are shortened for space.}
\label{tab:human_llm_examples}
\end{table}


==> tables/logit_lens_summary.tex <==
\begin{table}[t]
\centering
\scriptsize
\begin{tabular}{lcccc}
\toprule
Model & Layers & Mean logprob (first) & Mean logprob (last) \\
\midrule
Llama-3.1-70B & 0--80 & -47.59 & -21.46 \\
Qwen2.5-32B & 0--64 & -48.26 & -17.64 \\
\bottomrule
\end{tabular}
\caption{Logit-lens summary (20 puzzles). Mean reference-move logprob (Lichess solution) at the first and last layer.}
\label{tab:logit_lens_summary}
\end{table}


==> tables/masking_audit.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lrr}
\toprule
Mask & Audited & Residual leakage \\
\midrule
Light & 60 & .567 \\
Strict & 60 & .567 \\
Coordinates & 60 & .567 \\
Maximal & 60 & .000 \\
\bottomrule
\end{tabular}
\caption{Automatic masking audit on 60 sampled explanations. The residual detector flags UCI/SAN, coordinates, piece--square phrases, and promotion language. Maximal masking removes all audited leakage classes.}
\label{tab:masking_audit}
\end{table}


==> tables/motif_effects.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{llrrr}
\toprule
Type & Expected motif & $n$ & Exact & Gen.\ rec. \\
\midrule
Pawn & absent & 27 & .111 & .259 \\
 & present & 93 & .140 & .548 \\
Rook & absent & 35 & .143 & .400 \\
 & present & 130 & .092 & .520 \\
Bishop & absent & 16 & .063 & .250 \\
 & present & 24 & .000 & .261 \\
Knight & absent & 4 & .000 & .250 \\
 & present & 26 & .077 & .231 \\
\bottomrule
\end{tabular}
\caption{Move correctness and generated-move recoverability conditional on mentioning an expected endgame motif. Counts are explanation rows, not unique puzzles.}
\label{tab:motif_effects}
\end{table}


==> tables/predictive_selected.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{llrr}
\toprule
Outcome & Standardized predictor & Coefficient & Bootstrap 95\% interval \\
\midrule
Correct move & Reference-move rank & $-.978$ & $[-1.552,-.547]$ \\
Correct move & Square mentions & $-.616$ & $[-1.279,-.040]$ \\
Generated recovery & Legal generated move & $.403$ & $[.136,.652]$ \\
Generated recovery & Clipped engine loss & $-.371$ & $[-.715,-.169]$ \\
Reference recovery & Generated move correct & $1.109$ & $[.835,1.585]$ \\
Generated recovery & Expected motif mentioned & $.128$ & $[-.102,.405]$ \\
\bottomrule
\end{tabular}
\caption{Selected coefficients from exploratory logistic classifiers with puzzle-clustered bootstrap intervals. Models also include length, specificity, prompt, rating, material, theme, endgame type, and endgame--motif interactions. Coefficients are descriptive rather than causal.}
\label{tab:predictive_selected}
\end{table*}


==> tables/prob_recoverability_by_margin.tex <==
\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc}
\toprule
Margin bucket & $n$ & Recoverability & Mean $\Delta$ (cp) \\
\midrule
-5 to -2 & 146 & 0.321 & 10190.0 \\
>=-0.5 & 136 & 0.351 & 13695.5 \\
< -5 & 242 & 0.354 & 13014.5 \\
-2 to -0.5 & 64 & 0.381 & 8920.5 \\
\bottomrule
\end{tabular}
\caption{Recoverability by reference-vs-top logprob margin bucket. Margin is reference logprob minus top logprob (closer to 0 = more internal uncertainty).}
\label{tab:prob_recoverability_margin}
\end{table}


==> tables/prob_recoverability_by_rank.tex <==
\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc}
\toprule
Reference rank & $n$ & Recoverability & Mean $\Delta$ (cp) \\
\midrule
2-3 & 191 & 0.321 & 11192.7 \\
1 & 113 & 0.352 & 14443.0 \\
4-5 & 172 & 0.412 & 12272.2 \\
>5 & 112 & 0.297 & 10501.3 \\
\bottomrule
\end{tabular}
\caption{Recoverability by reference-move rank bucket (Mistral-7B token-prob scoring; brief prompt).}
\label{tab:prob_recoverability_rank}
\end{table}


==> tables/qwen32b_scoring_controls.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{llcccc}
\toprule
Prompt & Scoring context & Ref.@1 & Ref.@3 & Gen.@1 & Gen.@3 \\
\midrule
Brief & FEN only & .16 & .42 & .08 & .22 \\
 & FEN + maximal mask & .14 & .36 & .12 & .30 \\
 & FEN + unmasked & .18 & .36 & .50 & .52 \\
 & FEN + random explanation & .06 & .26 & .06 & .20 \\
\midrule
Calculation & FEN only & .18 & .40 & .10 & .16 \\
 & FEN + maximal mask & .18 & .42 & .10 & .20 \\
 & FEN + unmasked & .12 & .38 & .40 & .42 \\
 & FEN + random explanation & .04 & .22 & .04 & .16 \\
\midrule
Teaching & FEN only & .16 & .36 & .10 & .22 \\
 & FEN + maximal mask & .16 & .36 & .14 & .34 \\
 & FEN + unmasked & .14 & .36 & .60 & .60 \\
 & FEN + random explanation & .14 & .30 & .08 & .26 \\
\bottomrule
\end{tabular}
\caption{Qwen2.5-32B all-legal-move scoring on 50 puzzles. Ref.\ and Gen.\ denote ranks of the reference and generated moves. Unmasked explanations are an upper-bound leakage check; random explanations come from another puzzle under the same prompt style.}
\label{tab:qwen32b_controls}
\end{table*}


==> tables/recoverability_targets.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{lccccc}
\toprule
Prompt & $n$ & Generated@1 & Generated@3 & Reference@1 & Reference@3 \\
\midrule
Brief & 191 & .398 [.330,.466] & .518 [.450,.592] & .058 [.026,.094] & .099 [.058,.147] \\
Calculation & 195 & .379 [.313,.446] & .462 [.390,.533] & .056 [.026,.092] & .103 [.062,.149] \\
Teaching & 197 & .391 [.325,.462] & .503 [.431,.574] & .091 [.056,.132] & .137 [.091,.188] \\
\bottomrule
\end{tabular}
\caption{Top-1 and top-3 recoverability under strict masking, with puzzle-bootstrap 95\% intervals. Generated recovery targets the move produced by GPT-4.1-mini; reference recovery targets the Lichess solution move.}
\label{tab:recoverability_targets}
\end{table*}


==> tables/tokenprob_ablation_llama70b.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lcccccc}
\toprule
Prompt & Top-1 & Top-3 & Top-5 & Mean rank & Median rank & Mean $\Delta$ (ref-top) \\
\midrule
scoring\_only & 0.285 & 0.575 & 0.770 & 3.35 & 3.00 & -2.14 \\
\bottomrule
\end{tabular}
\caption{Token-probability ablation for Llama-3.1-70B (4-bit). $\Delta$ is reference logprob minus top-prob logprob.}
\label{tab:tokenprob_ablation_llama70b}
\end{table*}


==> tables/tokenprob_ablation_qwen32b.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lcccccc}
\toprule
Prompt & Top-1 & Top-3 & Top-5 & Mean rank & Median rank & Mean $\Delta$ (ref-top) \\
\midrule
scoring\_only & 0.245 & 0.555 & 0.780 & 3.46 & 3.00 & -2.06 \\
\bottomrule
\end{tabular}
\caption{Token-probability ablation for Qwen2.5-32B. $\Delta$ is reference logprob minus top-prob logprob.}
\label{tab:tokenprob_ablation_qwen32b}
\end{table*}


==> tables/tokenprob_ablation_qwen32b_expl.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lcccccc}
\toprule
Prompt & Top-1 & Top-3 & Top-5 & Mean rank & Median rank & Mean $\Delta$ (ref-top) \\
\midrule
brief & 0.175 & 0.490 & 0.745 & 3.73 & 4.00 & -4.41 \\
calc & 0.205 & 0.525 & 0.740 & 3.65 & 3.00 & -4.51 \\
teaching & 0.190 & 0.525 & 0.750 & 3.64 & 3.00 & -4.51 \\
\bottomrule
\end{tabular}
\caption{Token-probability ablation for Qwen2.5-32B with explanation-conditioned scoring (explanations masked).}
\label{tab:tokenprob_ablation_qwen32b_expl}
\end{table*}


==> tables/tokenprob_ablation_summary.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{lcccccc}
\toprule
Prompt & Top-1 & Top-3 & Top-5 & Mean rank & Median rank & Mean $\Delta$ (ref-top) \\
\midrule
brief & 0.215 & 0.540 & 0.820 & 3.46 & 3.00 & -3.70 \\
calc & 0.200 & 0.535 & 0.800 & 3.52 & 3.00 & -5.34 \\
teaching & 0.175 & 0.490 & 0.805 & 3.64 & 4.00 & -5.41 \\
\bottomrule
\end{tabular}
\caption{Token-probability ablation: reference-move rank under style-conditioned scoring prompts (open-weights model). $\Delta$ is reference logprob minus top-prob logprob; more negative means the reference move is less preferred.}
\label{tab:tokenprob_ablation}
\end{table*}

